Measuring Information Diffusion in Code Review at Spotify

Background: As a core practice in software engineering, the nature of code review has been frequently subject to research. Prior exploratory studies found that code review, the discussion around a code change among humans, forms a communication network that enables its participants to exchange and spread information. Although popular in software engineering, there is no confirmatory research corroborating this theory and the actual extent of information diffusion in code review is not well understood. Objective: In this registered report, we propose an observational study to measure information diffusion in code review to test the theory of code review as communication network. Method: We approximate the information diffusion in code review through the frequency and the similarity between (1) human participants, (2) affected components, and (3) involved teams of linked code reviews. The measurements approximating the information diffusion in code review serve as a foundation for falsifying the theory of code review as communication network.

==> tikz-hypergraph.tex <==
% Needs
% \usetikzlibrary{calc}
% \usepackage{ifthen}

\def\rotateclockwise#1{
  % Rotate input point by 90 degrees clockwise.
  \newdimen\xrw
  \pgfextractx{\xrw}{#1}
  \newdimen\yrw
  \pgfextracty{\yrw}{#1}
  % \pgfpoint{-\y}{\x}
  \pgfpoint{\yrw}{-\xrw}
}

\def\rotatecounterclockwise#1{
  % Rotate input point by 90 degrees clockwise.
  \newdimen\xrcw
  \pgfextractx{\xrcw}{#1}
  \newdimen\yrcw
  \pgfextracty{\yrcw}{#1}
  % \pgfpoint{-\y}{\x}
  \pgfpoint{-\yrcw}{\xrcw}
}

\def\outsidespacerpgfclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (clockwise)
  % to the vector from start point to end point.
  \pgfpointscale{#3}{
    \rotateclockwise{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\outsidespacerpgfcounterclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Compute a length-radius vector perpendicular (counterclockwise)
  % to the line from start point to end point.
  \pgfpointscale{#3}{
    \rotatecounterclockwise{
      \pgfpointnormalised{
        \pgfpointdiff{#1}{#2}}}}
}

\def\outsidepgfclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\outsidespacerpgfclockwise{#1}{#2}{#3}}
}

\def\outsidepgfcounterclockwise#1#2#3{
  % #1 start point
  % #2 end point
  % #3 radius
  % Add to end point a length-radius vector perpendicular
  % (counter-clockwise) to the line from start point to end point.
  \pgfpointadd{#2}{\outsidespacerpgfcounterclockwise{#1}{#2}{#3}}
}

\def\outside#1#2#3{
  ($ (#2) ! #3 ! -90 : (#1) $)
}

\def\cornerpgf#1#2#3#4{
  % #1 = previous pgf point 
  % #2 = current pgf point
  % #3 = next pgf point
  % #4 = radius
  % Computes a path comprising a rounded corner on the outside of the angle #1#2#3.
  \pgfextra{
    \pgfmathanglebetweenpoints{#2}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
    \let\anglea\pgfmathresult
    \let\startangle\pgfmathresult

    \pgfmathanglebetweenpoints{#2}{\outsidepgfclockwise{#3}{#2}{#4}}
    \pgfmathparse{\pgfmathresult - \anglea}
    \pgfmathroundto{\pgfmathresult}
    \let\arcangle\pgfmathresult
    \ifthenelse{180=\arcangle \or 180<\arcangle}{
      \pgfmathparse{-360 + \arcangle}}{
      \pgfmathparse{\arcangle}}
    \let\deltaangle\pgfmathresult

    \newdimen\x
    \pgfextractx{\x}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
    \newdimen\y
    \pgfextracty{\y}{\outsidepgfcounterclockwise{#1}{#2}{#4}}
  }
  -- (\x,\y) arc [start angle=\startangle, delta angle=\deltaangle, radius=#4]
}

\def\corner#1#2#3#4{
  \cornerpgf{\pgfpointanchor{#1}{center}}{\pgfpointanchor{#2}{center}}{\pgfpointanchor{#3}{center}}{#4}
}


\def\hedgeiii#1#2#3#4{
  % #1#2#3 = tikz points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the
  % convex hull H of the points #1#2#3 that have distance #4 to H.
  % Points #1#2#3 need to be in clockwise order.
  \outside{#1}{#2}{#4} \corner{#1}{#2}{#3}{#4} \corner{#2}{#3}{#1}{#4} \corner{#3}{#1}{#2}{#4} -- cycle
}

\def\hedgem#1#2#3#4{
  % #1#2 = tikz points
  % #3 = list of tikz points
  % #4 = radius
  % Computes a path comprising the line of the points outside of the convex hull H of the points #1#2[#3] that have distance #4 to H.
  % Points #1#2[#3] need to be vertices of a convex polygon and in clockwise order.
  
  \outside{#1}{#2}{#4}
  \pgfextra{
    \def\hgnodea{#1}
    \def\hgnodeb{#2}
  }
  foreach \c in {#3} {
    \corner{\hgnodea}{\hgnodeb}{\c}{#4}
    \pgfextra{
      \global\let\hgnodea\hgnodeb
      \global\let\hgnodeb\c
    }
  }
  \corner{\hgnodea}{\hgnodeb}{#1}{#4}
  \corner{\hgnodeb}{#1}{#2}{#4}
  -- cycle
}

\def\hedgeii#1#2#3{
  % #1#2 = tikz points
  % #3 = radius
  \hedgem{#1}{#2}{}{#3}
}

\def\hedgei#1#2{
  % #1 = tikz point
  % #2 = radius
  (#1) circle [radius = #2]
}
